Crowdsourcing Relative Rankings of Multi-Word Expressions: Experts versus Non-Experts

In this study we investigate to which degree experts and non-experts agree on questions of difficulty in a crowdsourcing experiment. We ask non-experts (second language learners of Swedish) and two groups of experts (teachers of Swedish as a second/foreign language and CEFR experts) to rank multi-word expressions in a crowdsourcing experiment. We find that the resulting rankings by all the three tested groups correlate to a very high degree, which suggests that judgments produced in a comparative setting are not influenced by professional insights into Swedish as a second language.

==> reviewer_checklist.tex <==
% Reviewer checklist for Language Learning
% Specifically for Methods Showcase Articles

1. Focuses on an emerging or a new method that is or could be relevant to language learning research

2. Provides a strong overview of the method’s details

3. Compares method to more traditional approaches

4. Provides a replicable application of the method

5. Provides information about good reporting practices for the method

6. Provides information about appropriate and clear interpretations/claims that can be made using the method

7. Provides open access to the method

8. Provides open access to the data used as proof of concept

9. Discusses the method’s limitations

10. Provides alternatives to method if available

11. Is of the proper length (~8,000 words in total)

12. Contains accessible writing 

==> sections/unused_things.tex <==

%==================================================


intro about crowdsourcing as a method in language learning/resource building method 

Research questions
1. (Can crowdsourcing be used as a method for creating/preparing second language learning material?)

2. Does the voter background influence the vote?
%Do learners and teachers agree with each other? (intuition-based / based on ranking)
%Do “experts” agree with teachers? With learners?
(2.1) Can non-experts be trusted?

Does the number of votes change the picture a lot or not? 
— by group of voters, across, mixed (random)

Time for annotation

%Do experts agree with themselves when directly annotating vs when ranking?

Which type of (CEFR-)level assignment is to be trusted? 
Do learners/teachers/experts agree with L2 corpora authors - by group and jointly?
Do learners/teachers/experts agree with General corpora statistics - by group and jointly?

% future work
Could the same methods of level-linking  apply to other types of lexical items (e.g. single items)?

%=======================

CS has been used like this and that, and they have all wondered whether background influences

Prove that subjective judgements are on-par with expert knowledge (Kasperowski)

%====

The problem:
data and resources+
how to address different learners at different levels
create resources using crowd
exploring now 

does the corpus give us a correct picture of levels?
could it be complemented?

test CS as a method for unordered list of items (for L2)
find natural way of ordering/assessing materials
compare to EVP

problem not solved wrt level assignment
only relative ranking

outliers

==
rename idioms to -> ??

description of experiment

add expert direct labeling
Î
time for annotation

this is method analysis

practical implications

use cs with mixed crowd given unordered list that we are interested in using in teaching

compare costs?

%============
future work

clustering into levels
use anchors with known levels -> cluster around them
as practical application of deriving levels

maybe split into levels
representative vocabulary of each level (let us assume we have X of known, and add Y unknown, that would mean that ... we need A votes and would take B time) % TODO calculate for 10+10 items, minimum amount of votes => 20 items => 36 combinations
% => 2 crowdsourcers, 30 seconds per task, number of responses 3: 27 min
% => 2 crowdsourcers, 30 seconds per task, number of responses 3: 18 min
how does other vocabulary cluster around
needs to be tested

chapter on experiment


%==> conclusion
in this context, crowds are not different
this can help build language learning resources without considering background

HYP: given unordered list of items and using CS, => ordered scale => use for language teaching, analysis of language learning

SETUP:
as-is, no comparison to coctaill

METHODOLOGY:

%===============

\pgfplotsset{every axis/.append style={thick, tick style=semithick}}

\begin{figure}
\pgfplotstableread[col sep=comma,]{plot_data/dist_age.csv}\distage
\begin{tikzpicture}

\begin{axis}[
    ybar,
    bar width=.9cm,
    width=\textwidth,
    height=10cm,
    ymin = 0,
    xtick=data,
    xticklabels from table={\distage}{Years},
    x tick label style={font=\normalsize, rotate=90},
    ylabel={Count}
    ]
    \addplot [] table [x expr=\coordindex, y={Count}]{\distage};
\end{axis}
\end{tikzpicture}
\end{figure}

\begin{figure}
\pgfplotstableread[col sep=comma,]{plot_data/dist_gender.csv}\distgender
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=1cm,
    width=\textwidth,
    height=10cm,
    ymin=0,
    xtick=data,
    xticklabels from table={\distgender}{Gender},
    x tick label style={font=\normalsize},
    ylabel={Count}
    ]
\addplot [] table [x expr=\coordindex, y={Count}]{\distgender};
\end{axis}
\end{tikzpicture}
\end{figure}


\begin{figure}
    \centering
    \pgfplotstableread[col sep=comma,]{plot_data/dist_prof.csv}\distprof
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=1cm,
        width=\textwidth,
        height=10cm,
        ymin=0,
        xtick=data,
        xticklabels from table={\distprof}{Proficiency},
        x tick label style={font=\normalsize},
        ylabel={Count}
    ]
    \addplot [] table [x expr=\coordindex, y={Count}]{\distprof};
    \end{axis}
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \pgfplotstableread[col sep=comma,]{plot_data/dist_res.csv}\distres
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=1cm,
        width=\textwidth,
        height=10cm,
        ymin=0,
        xtick=data,
        xticklabels from table={\distres}{Country},
        x tick label style={font=\normalsize},
        ylabel={Count}
    ]
    \addplot [] table [x expr=\coordindex, y={Count}]{\distres};
    \end{axis}
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}




k-means confusion matrix


[8, 2, 2, 0, 0]
[1, 8, 2, 1, 0]
[1, 4, 4, 3, 0]
[0, 2, 2, 8, 0]
[0, 5, 3, 4, 0]

spectral confusion matrix

[10, 0, 2, 0, 0]
[4, 5, 3, 0, 0]
[1, 3, 5, 3, 0]
[1, 2, 2, 7, 0]
[2, 4, 3, 3, 0]

k-means confusion matrix

[10, 2, 0, 0, 0]
[6, 3, 1, 0, 2]
[4, 1, 5, 0, 2]
[3, 0, 5, 0, 4]
[1, 0, 5, 0, 6]

spectral confusion matrix

[7, 5, 0, 0, 0]
[3, 7, 0, 0, 2]
[1, 4, 5, 0, 2]
[0, 5, 3, 0, 4]
[0, 2, 3, 0, 7]

k-means confusion matrix

[7, 2, 3, 0, 0]
[2, 7, 2, 0, 1]
[0, 6, 4, 0, 2]
[0, 6, 1, 0, 5]
[0, 3, 1, 0, 8]

spectral confusion matrix

[8, 0, 2, 1, 1]
[2, 0, 5, 2, 3]
[0, 0, 9, 2, 1]
[0, 0, 2, 7, 3]
[0, 0, 1, 2, 9]



\begin{figure}
    \centering
    
    \begin{tikzpicture}
    \node (Z) at (5,5) {$l_1$};
    \node (Y) at (10,5) {$l_2$};
    
    \node (X) at (2,0) {Least frequent};
    \node (W) at (2,4) {Most frequent};
    
    \node (S) at (13,5) {Score};
    
    \node (G) at (5,4) {$A$};
    \node (H) at (10,4) {$D$};
    \node at (13,4) {3};
    
    \node (A) at (5,3) {$B$};
    \node (B) at (10,3) {$A$};
    \node at (13,3) {1};
    
    \node (C) at (5,2) {$C$};
    \node (D) at (10,2) {$C$};
    \node at (13,2) {0};
    
    \node (E) at (5,1) {$D$};
    \node (F) at (10,1) {$B$};
    \node at (13,1) {2};
    
    \draw (A) -- (B);
    \draw (C) -- (D);
    \draw (E) -- (F);
    \draw (G) -- (H);
    \end{tikzpicture}
    \caption{Out-of-place metric illustration}
    \label{fig:oop:illustration}
\end{figure}


To add? Mother tongues, other languages

% YOB

Average time for L2 learners vs teachers ve experts
Info about number of votes
Problems (parallel experiments, setup, finished items, …)
Include the link to the open crowd: %https://ws.spraakbanken.gu.se/ws/tools/crowd-tasking/project/l2p_mwe_group2_other/

Total amount of annotators per category

Time per task per annotator
Annotator 11: 
Group 1 39.94 seconds
Group 2 44.92 seconds
Group 3 Average 27.36 seconds per task

Annotator 24:
Group 1 28.63 s
Group 2 23.78 s
Group 3 21.71 s
Annotator46
Group 1 28.75

Group 2 36.73

Group 3 60.26


Average annotator: 
Group 1 32.44
Group 2 35.14
Group 3 36.44


Total time per annotator per project:
G1
11 3:37:00.692384
24 2:35:33.399893
46 2:36:12.064365
G2
11 3:45:43.411272
24 2:09:10.840639
46 3:19:35.321276

G3
11 2:28:40.732774
24 1:57:56.260348
46 5:27:26.089252





